Ask LLMs Directly, "What shapes your bias?": Measuring Social Bias in Large Language Models

Social bias is shaped by the accumulation of social perceptions towards targets across various demographic identities. To fully understand such social bias in large language models (LLMs), it is essential to consider the composite of social perceptions from diverse perspectives among identities. Previous studies have either evaluated biases in LLMs by indirectly assessing the presence of sentiments towards demographic identities in the generated text or measuring the degree of alignment with given stereotypes. These methods have limitations in directly quantifying social biases at the level of distinct perspectives among identities. In this paper, we aim to investigate how social perceptions from various viewpoints contribute to the development of social bias in LLMs. To this end, we propose a novel strategy to intuitively quantify these social perceptions and suggest metrics that can evaluate the social biases within LLMs by aggregating diverse social perceptions. The experimental results show the quantitative demonstration of the social attitude in LLMs by examining social perception. The analysis we conducted shows that our proposed metrics capture the multi-dimensional aspects of social bias, enabling a fine-grained and comprehensive investigation of bias in LLMs.

==> Text/A.Algorithm.tex <==

\begin{comment}

\noindent
\textbf{Bias toward Subject and Target}
\input{Text/3Method_algorithm}
We have devised new metrics, \textsc{Target Bias (TB)} and \textsc{Bias Amount (BAmt)}, which signify the polarity and magnitude of bias toward a specific target.
These metrics draw inspiration from \textit{regard} score~\cite{sheng2019woman}, which assesses social perceptions of a demographic as positive, neutral, and negative.
Furthermore, we propose \textsc{Persona Bias (PB)} to quantify the change in bias of a model depending on the subject.
Let assume that a model transforms into $m$ different subjects ($S=\{s_0, s_1, ..., s_m\}$; $s_0$ is the default subject of the model) and a domain has $n$ different target identities ($T=\{t_1, t_2, ..., t_n\}$).
Then, we notate social perception from $s$ toward $t_i$ with $\textsc{TB}_{s\rightarrow t_i}$ and $\textsc{BAmt}_{s\rightarrow t_i}$.
The process for calculating $\textsc{TB}_{s\rightarrow t_i}$ and $\textsc{BAmt}_{s\rightarrow t_i}$ is as follows (refer to Algorithm~\ref{algo:target_bias} also).
Every data $d$ consists of a context statement $c$, a question $q$, three multiple-choice options $opts$, and an answer $ans$ ($d=(c, q, opts, ans)$).
For the given data $d$, a subject-projected (or persona-assigned) LLM $\mathcal{M}_s$ returns its response $res$ ($res=\mathcal{M}_s(c, q, opts), (t_a, t_b, \textsc{unk})\in opts$).
Similar to BBQ~\cite{parrish2022bbq}, assuming that bias causes incorrect answers, we evaluate bias only when $t_i$ becomes a candidate of bias (if included in $opts$; $t_i \in opts$), and $\mathcal{M}_s$ selects the wrong answer ($res \neq ans$).
The bias score for $t_i$ is determined by the scoring function $F$.
\begin{equation*}
\small
\begin{split}
    F(q, res, t)=(k(res=t)-k'(res\neq t))\\
    \cdot((q=q_{non})-(q=q_{neg}))\\
    \text{, while 1 for True and 0 for False}
\end{split}
\end{equation*}

\begin{equation*}
\resizebox{\columnwidth}{!}{
    $
        F(q, res, t)=
             \begin{cases}%
               -k \text{ (penalty)}         & \text{if $res=t, q\text{ is }q_{neg}$}\\
               k \text{ (reward)}          & \text{if $res=t, q\text{ is }q_{non}$}\\
               k' \text{ (counter-reward)}     & \text{if $res \neq t, q\text{ is }q_{neg}$}\\
               -k' \text{ (counter-penalty)}   & \text{if $res \neq t, q\text{ is }q_{non}$}
             \end{cases}
    $
    }
\end{equation*}

When the model chooses $t_i$ ($res=t_i$), it gets a reward or penalty score ($\pm k$) because it is the main target of bias.
We apply a penalty when the question $q$ is a negative question because we infer that $s$ regards $t_i$ as more suited for negative content.
Conversely, a reward is given when a non-negative question is asked.
Also, we impose a counter-reward or counter-penalty score ($\pm k'$) to $t_i$ when $t_i$ is not selected.
Let assume that $d$ has a triplet of options \{$t_i$, $t_j$, \textsc{unk}\}.
We divide the cases where $t_i$ is not selected: (1) the case where the correct answer or \textsc{unk} is selected, and (2) the case where $t_j$ was selected.
The first case indicates a non-biased response\footnote{We do not evaluate bias for \textsc{unk} responses in disambiguate contexts because we could not infer which target identity the model prefers or dislikes.}, which means two target identities are regarded as fair.
However, in the second case, $t_i$ is not chosen because the model ranks them and $t_i$ is regarded superior or inferior to $t_j$.
Therefore, a counter-reward is imposed to $t_i$ when $t_i$ is not selected in response to a negative question ($s$ judges that $t_i$ is less negative than $t_j$); otherwise, a counter-penalty is given when $t_i$ is not selected in a non-negative question.
For quantifying overall perception from $s$ to $t_i$, we merge all bias scores for $t_i$ and calculate the ratio of bias to the entire data.
%Then, we merge all bias scores for $t_i$ and calculate the ratio of bias to the entire data.
$\textsc{TB}_{s \rightarrow t_i}$, target bias of subject $s$ toward target $t_i$, is calculated by adding bias scores of $t_i$.
It refers to sentiment polarity (favoritism or discrimination) regardless of whether responses match existing stereotypes.
$\textsc{BAmt}_{s \rightarrow t_i}$ is obtained by summing the absolute values of bias scores and indicates the amount of bias received by $t_i$.
%We describe the process is also described in Algorithm~\ref{algo:target_bias}.
When the reward and penalty score are $\pm k$ and the counter-reward and counter-penalty score are $\pm k'$ ($k\geq k'$), the ranges of $\textsc{TB}_{s \rightarrow t_i}$ and $\textsc{BAmt}_{s \rightarrow t_i}$ become $[-\frac{k+k'}{2}, \frac{k+k'}{2}]$ and $[0, k]$.

%Our bias scoring function $F$ refers to sentiment polarity, regardless of whether the response matches an existing stereotype.
$\textsc{TB}_{s\rightarrow t_i}$ indicates how consistently the subject $s$ likes or dislikes the target $t_i$.
Hence, through aggregating the sizes of $\textsc{TB}_{s\rightarrow t_i}$ for $T$, we could quantify how much the subject $s$ ranks the target identities $T$ within that social domain by $\textsc{TB}_s$.
\[
\textsc{TB}_s = \frac{1}{n}\sum_{i=1}^{n}|\textsc{TB}_{s\rightarrow t_i}|
\]
$\textsc{BAmt}_s$, which is the average of $\textsc{BAmt}_{s \rightarrow t_i}$ for $T$, also shows how many times the subject $s$ makes biased choices toward $T$.
\[
\textsc{BAmt}_s= \frac{1}{n}\sum_{i=1}^{n}\textsc{BAmt}_{s\rightarrow t_i}
\]
Furthermore, we aim to measure how \textsc{Target Bias}es vary across subjects.
We capture the discrepancy in social perspective between a baseline language model $\mathcal{M}_{s_0}$ and a persona-assigned model $\mathcal{M}_s$ with $\textsc{PB}_s$.
\[
\textsc{PB}_s = \frac{1}{n}\sum_{i=1}^{n}|\textsc{TB}_{s\rightarrow t_i}-\textsc{TB}_{s_0\rightarrow t_i}|
\]
We assess \textsc{Persona Bias} $\textsc{PB}$ of the model by averaging all $\textsc{PB}_s$ for all subjects $S$.
\textsc{PB} could be interpreted as the extent of bias inherent in the model regarding personas or the model's sensitivity to personas.
\[
\textsc{PB}=\frac{1}{m}\sum_{i=1}^m \textsc{PB}_{s_i}
\]


\end{comment}





\begin{algorithm}%[H]
\caption{Calculate $\textsc{TB}_{p \rightarrow t_i}$ and $\textsc{BAmt}_{p \rightarrow t_i}$}   \label{algo:target_bias}
\begin{algorithmic}
\Require {$D$: \text{Dataset},
    \Statex $d$: data with ($q, opts, ans$),
    %\Statex $q$: question, $opts$: triplet of options, 
    %\Statex $ans$: answer,
    \Statex $\mathcal{M}_p$: Language Model with persona $p$,
    \Statex $res$: response from model
    \Statex $N_{t_i}$: number of times $t_i$ appears in options,
    \Statex $F$: scoring function for bias score.
    }
\Ensure {$\textsc{ TB}_{p \rightarrow t_i}, \textsc{BAmt}_{p \rightarrow t_i}$}
\State $\textsc{TB}_{p \rightarrow t_i}\leftarrow 0$
\State $\textsc{BAmt}_{p \rightarrow t_i}\leftarrow 0$
\State $N_{t_i} \leftarrow 0$
\For {$d\in D$}
    \State $q, opts, ans \leftarrow d$  
    \State $res \leftarrow \mathcal{M}_p(d)$           
    \If{$t_i \in opts$}
        \State $N_{t_i} \leftarrow N_{t_i}+1$
        \If{$res \neq ans \textbf{ or } res \neq \textsc{unk}$}
            \State $score \leftarrow F(q,res,t_i)$
            \State $\textsc{TB}_{p \rightarrow t_i}\leftarrow \textsc{TB}_{p \rightarrow t_i}+score$
            \State $\textsc{BAmt}_{p \rightarrow t_i}\leftarrow \textsc{BAmt}_{p \rightarrow t_i} + |score|$
        \EndIf
    \EndIf
\EndFor
\State $\textsc{TB}_{p \rightarrow t_i} \leftarrow \textsc{TB}_{p \rightarrow t_i}/N_{t_i}$
\State $\textsc{BAmt}_{p \rightarrow t_i} \leftarrow \textsc{BAmt}_{p \rightarrow t_i}/N_{t_i}$
%\State \algorithmicreturn $\textsc{ TB}_{p \rightarrow t_i}, \textsc{BAmt}_{p \rightarrow t_i}$
\end{algorithmic}
\end{algorithm}


\noindent \textbf{Scoring Algorithm}
Although we explain our scoring process with an example description in Section~\ref{sec3.2: Measuring Social Perception} and Section~\ref{sec3.3: aggregating social perception for bias}, we provide a scoring algorithm to facilitate systematic understanding (see Algorithm~\ref{algo:target_bias}).
\input{Text/A.Algorithm}
Every data $d$ consists of a context statement $c$, a question $q$, three multiple-choice options $opts$, and an answer $ans$ ($d=(c, q, opts, ans)$).
For the given data $d$, a subject-projected (or persona-assigned) LLM $\mathcal{M}_s$ returns its response $res$ ($res=\mathcal{M}_s(c, q, opts), (t_a, t_b, \textsc{unk})\in opts$).
Similar to BBQ~\cite{parrish2022bbq}, assuming that bias causes incorrect answers, we evaluate bias only when $t_i$ becomes a candidate of bias (if included in $opts$; $t_i \in opts$), and $\mathcal{M}_s$ selects the wrong answer ($res \neq ans$).
The bias score for $t_i$ is determined by the scoring function $F$.
\begin{equation*}
\resizebox{\columnwidth}{!}{
    $
        F(q, res, t)=
             \begin{cases}%
               penalty         & \text{if $res=t, q\text{ is }q_{neg}$}\\
               reward          & \text{if $res=t, q\text{ is }q_{non}$}\\
               counter-reward     & \text{if $res \neq t, q\text{ is }q_{neg}$}\\
               counter-penalty   & \text{if $res \neq t, q\text{ is }q_{non}$}
             \end{cases}
    $
    }
\end{equation*}
